Fair clustering via equitable group representations

What does it mean for a clustering to be fair? One popular approach seeks to ensure that each cluster contains groups in (roughly) the same proportion in which they exist in the population. The normative principle at play is balance: any cluster might act as a representative of the data, and thus should reflect its diversity. But clustering also captures a different form of representativeness. A core principle in most clustering problems is that a cluster center should be representative of the cluster it represents, by being "close" to the points associated with it. This is so that we can effectively replace the points by their cluster centers without significant loss in fidelity, and indeed is a common "use case" for clustering. For such a clustering to be fair, the centers should "represent" different groups equally well. We call such a clustering a group-representative clustering. In this paper, we study the structure and computation of group-representative clusterings. We show that this notion naturally parallels the development of fairness notions in classification, with direct analogs of ideas like demographic parity and equal opportunity. We demonstrate how these notions are distinct from and cannot be captured by balance-based notions of fairness. We present approximation algorithms for group representative $k$-median clustering and couple this with an empirical evaluation on various real-world data sets.

==> ex_table.tex <==
\begin{table*}[]
\caption{Clustering Bank and Census datasets using LS-Fair and LP-Fair algorithms}
\label{ta:heuristic}
\centering
\resizebox{1.5\columnwidth}{!}{%
\begin{tabular}{@{}llcccccccc@{}}
\toprule
\multicolumn{2}{l}{\multirow{2}{*}[-0.25em]{Datasets}} & \multicolumn{2}{c}{\textit{1:1 Census}} & \multicolumn{2}{c}{\textit{1:5 Census}} & \multicolumn{2}{c}{\textit{1:1 Bank}} & \multicolumn{2}{c}{1:5 Bank} \\ \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} 
\multicolumn{2}{c}{} & female & male & female & male & married & single & married & single \\ \midrule
\multicolumn{2}{l}{Group optimal} & 34499 & 31528 & 35349 & 32619 & 569 & 686 & 659 & 655 \\ \addlinespace[5pt]
\multicolumn{2}{l}{Standard $k$-median} & 2.16 & 2.61 & 13.7 & 0.21 & 4.7 & 6.4 & 43.85 & 1.52 \\ \addlinespace[5pt]
\multirow{2}{*}{\error} & LS-Fair & 0.95 & 5.61 & 7.17 & 10.80 & 10.19 & 4.66 & 13.65 & 12.97 \\
 & LP-Fair & 0.48 & 7.74 & 8.61 & 9.36 & 10.72 & 4.51 & 12.29 & 16.48 \\ \addlinespace[5pt]
\multirow{2}{*}{\Ratio} & LS-Fair & 2.58 & 2.57 & 7.77 & 6.38 & 7.38 & 5.97 & 13.05 & 14.04 \\
 & LP-Fair & 2.60 & 2.58 & 7.68 & 3.81 & 7.73 & 5.24 & 16.38 & 13.43 \\ \bottomrule
\end{tabular}
}
\end{table*}



\begin{table*}[]
\caption{Clustering Bank and Census datasets using LS-Fair and LP-Fair algorithms}
\label{ta:heuristic}
\centering
\resizebox{1.5\columnwidth}{!}{%
\begin{tabular}{@{}llcccccccc@{}}
\toprule
\multicolumn{2}{l}{\multirow{2}{*}[-0.25em]{Datasets}} & \multicolumn{2}{c}{\textit{1:1 Census}} & \multicolumn{2}{c}{\textit{1:5 Census}} & \multicolumn{2}{c}{\textit{1:1 Bank}} & \multicolumn{2}{c}{1:5 Bank} \\ \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} 
\multicolumn{2}{c}{} & female & male & female & male & married & single & married & single \\ \midrule
\multicolumn{2}{l}{Standard $k$-median} & 35264 & 32351 & 40212 & 32689 & 596 & 730 & 948 & 665 \\ \addlinespace[5pt]
\multirow{2}{*}{\error} & LS-Fair & 34827 & 33298 & 37887 & 36144 & 627 & 718 & 749 & 740 \\
 & LP-Fair & 34668 & 33971 & 38396 & 35675 & 630 & 717 & 740 & 763 \\ \addlinespace[5pt] \midrule
 \multicolumn{2}{l}{Group optimal} & 34499 & 31528 & 35349 & 32619 & 569 & 686 & 659 & 655 \\ \addlinespace[5pt]
\multirow{2}{*}{\Ratio} & LS-Fair & 35390 & 32341 & 38099 & 34702 & 611 & 727 & 745 & 747 \\
 & LP-Fair & 35397 & 32343 & 38067 & 33865 & 613 & 722 & 767 & 743 \\ \bottomrule
\end{tabular}
}
\end{table*}


///////////////////////////

\begin{table*}[htbp]
\caption{Clustering Bank and Census datasets using LS-Fair and LP-Fair algorithms. Standard $k$-median and group optimal
rows present the actual groups’ average costs. \error and \Ratio rows are the percentage increase/decrease in group costs
for proposed algorithms, compared to the corresponding values in standard $k$-median and group optimal rows, respectively.}
\label{ta:heuristic}
\centering
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}llcccccccc@{}}
\toprule
\multicolumn{2}{l}{\multirow{2}{*}[-0.25em]{Datasets}} & \multicolumn{2}{c}{\textit{1:1 Census}} & \multicolumn{2}{c}{\textit{1:5 Census}} & \multicolumn{2}{c}{\textit{1:1 Bank}} & \multicolumn{2}{c}{1:5 Bank} \\ \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} 
\multicolumn{2}{c}{} & female & male & female & male & married & single & married & single \\ \midrule
\multicolumn{2}{l}{Standard $k$-median} & 35264 & 32351 & 40212 & 32689 & 596 & 730 & 948 & 665 \\ \addlinespace[5pt]
\multirow{2}{*}{\error (\%)} & LS-Fair & 98.7 & 102.9 & 94.2 & 110.5 & 105.2 & 98.3 & 79 & 111.2 \\
 & LP-Fair & 98.3 & 105 & 95.5 & 109.1 & 105.7 & 98.2 & 78 & 114.7 \\ \addlinespace[5pt] \midrule
 \multicolumn{2}{l}{Group optimal} & 34499 & 31528 & 35349 & 32619 & 569 & 686 & 659 & 655 \\ \addlinespace[5pt]
\multirow{2}{*}{\Ratio (\%)} & LS-Fair & 102.5 & 102.5 & 107.7 & 106.3 & 107.3 & 105.9 & 113 & 114 \\
 & LP-Fair & 102.6 & 102.5 & 107.6 & 103.8 & 107.7 & 105.2 & 116.3 & 113.4 \\ \bottomrule
\end{tabular}
%}
\end{table*}


\begin{table*}
\caption{Effects of enforcing balance on group representations}
\label{tab:balance}
%\resizebox{\columnwidth}{!}{
\centering
\begin{tabular}{@{}lcccccccc@{}}
\toprule
\multicolumn{1}{l}{\multirow{2}{*}[-0.25em]{Datasets}} & \multicolumn{2}{c}{Synthetic} & \multicolumn{2}{c}{Iris} & \multicolumn{2}{c}{Census} & \multicolumn{2}{c}{Bank} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
\multicolumn{1}{c}{}	&	majority	&	minority	&	Setosa    & Versicolor   & female       & male        & married     & single     \\ \midrule
Standard $k$-median	& 0.514		& 0.678		& 0.169     & 0.256        & 34492     & 35083    & 627      & 682     \\
Balanced $k$-median	& 0.430 	& 3.476		& 0.101     & 2.819        & 34019     & 35876    & 622      & 694     \\ \bottomrule
\end{tabular}
%}
\end{table*}

==> extra.tex <==
\section{$k$-Means Clustering}
Given $n$ data points $\{a_1,a_2,\dots,a_n\}$ in $\mathbb{R}^d$, $k$-means clustering aims to partition them into $k$ clusters, minimizing the sum of square Euclidean distances between each point and its nearest cluster center:
\[\sum_{i=1}^n \norm{a_i - \mu_{\mathcal{C}(a_i)}}_2^2\]
where $\mu_{\mathcal{C}(a_i)}$ is the center of the cluster $a_i$ is assigned to. $k$-means minimizes the sum of variances of the clusters. This problem can be relaxed into a more general case, namely $k$-rank approximation, where the goal is to find a subspace of rank at most $k$, which approximates the given data points best \citep{turning,cohen}. Given $n$ data points $\{a_1,a_2,\dots,a_n\}$ in $\mathbb{R}^d$ and set $\mathcal{S}$ of all rank $k$ orthogonal projections in $\mathbb{R}^{n\times n}$, $k$-rank approximation aims to find:
\[\argmin_{P \in \mathcal{S}} \norm{A-PA}^2_F\]
This relaxed version of the problem can be solved exactly in polynomial time, using singular value decomposition, as opposed to $k$-means clustering which is known to be NP-hard \cite{drineas2004clustering}. In this relaxation, the points representing cluster centers in $k$-means, are replaced by subspaces. Also, the cost of this clustering is the cost of projecting the points in the original space, onto the rank $k$ subspace. It is easy to see a lower-bound for the $k$-means problem is an upper-bound for the $k$-rank approximation, as any $k$ points (centers), can be contained in a subspace of rank at most $k$. Therefore, a solution to the $k$-means problem would naturally lead to a solution for $k$-rank approximation.

%\citep{turning} and \citep{cohen} study the problem of approximating a large high dimensional dataset $A$ in Euclidean space $R^d$, with a smaller sketch \~{A}. A solution to this problem can be useful in solving $k$-rank approximation problems such as $K$-Means Clustering to within a $(1+\epsilon)$ error. In both papers, the reduction only depends on some problem parameters (like the number of clusters, $K$) and the quality of the approximation ($\epsilon$), but not on the number of input items or the dimension of the input space. The main result in \citep{turning} is a dimensionality reduction algorithm for $n$ points in high $d$-dimensional space to $n$ points in $O(j/\epsilon^2)$ dimensional space, such that the sum of squared distances to every object that is contained in a $j$-dimensional subspace is approximated up to a $(1 + \epsilon)$-factor. One of the results from \citep{cohen}, improves the $O(k/\epsilon^2)$ rank approximation in \citep{turning} to $O(k/\epsilon)$.
%
%Both \citep{fairpca} and \citep{convex} study the problem of fair PCA. However, \citep{convex} consider a notion of fairness similar to \emph{disparate impact} with the idea that that a protected class cannot be inferred from the dimensionality-reduced data; while \citep{fairpca} take the equalized odds approach. Given a matrix $Y$ as dataset and and approximation $Z$ for it, \citep{fairpca} introduce the notion of \emph{Reconstruction Loss} as the difference between reconstruction error of $Y$ with respect to $Z$ and that of the best possible approximation for $Y$. The goal is to minimize the maximum Reconstruction Loss suffered by any group.


%\section{Fairness in clustering vs fairness in classification}
%Group fairness measures aside, I think both these notions satisfy individual fairness in a %sense. Consider two points with a distance less than $\epsilon$. We defined fairness as the %equality of distance between a point and its center (direction) and not the center itself. %So even if the two points are assigned to different centers, it's enough for the difference %between each point and its cluster center to be less than $\epsilon$ times a scalar. But we %know the said difference should be smaller than $\epsilon$ since otherwise, one of the %points should have been assigned to the other cluster center.

Samadi et al. proposed an algorithm which can be used to solve the $k$-rank approximation problem with loss-fair constraint \citep{fairpca}. Their algorithm relaxes the roblem to a semidefinite optimization problem later solves an LP designed to reduce the rank of SDP solution. In what follows, we redefine our proposed notions of fairness specifically for relaxed version of $k$-Means clustering, and present approximation ratios for each case, when the algorithm proposed by Samadi et al. is used to solve the problem.

\begin{defn} (Error). 
Given a matrix $Y$, error for matrix $X$ with rank at most $k$ which approximates $Y$, is defined as:
\[Error(Y,X) \coloneqq \norm{Y-X}^2_F\]
\end{defn}

\begin{defn}(Error-fair $k$-means). 
Given a set of data points partitioned into two groups $A$ and $B$, the problem of finding a fair $k$-rank approximation with respect to error, is defined as optimizing:
\[\argmin_{f: rank(f)\leq k} max\{\frac{1}{|A|}error(A,A^f),\frac{1}{|B|}error(B,B^f)\}\]
where $A^f$ is the projection of $A$ onto $f$.
\end{defn}

\begin{thm}
Let $f$ be solution to the error-fair $k$-means problem. Then:
\[\frac{1}{|A|}error(A,A^f) = \frac{1}{|B|}error(B,B^f)\]
\end{thm}
\begin{proof}
Refer to the proof of \ref{th:equal}.
\end{proof}

\begin{thm}
Given a set of data points $X \in \mathbb{R}^{m \times n}$, solving the $k$-means clustering problem on the projection of $X$ onto the error-fair subspace $f: rank(f) \leq k$, returns a $2+\frac{|A|}{|B|}$-approximate solution.
\label{th:error-fair}
\end{thm}

\begin{proof}
Cost of the solution returned by this algorithm, consists of two sets of distances: 1. sum of distances between each point and subspace $f$ (projection cost). 2. sum of distances between projection of each point onto $f$ and its cluster center in $f$. If $\mathcal{C} = \{C^1,C^2,\dots,C^k\}$ is an optimal solution to the problem in the original space, it is easy to see that:
\begin{equation}
Z = \sum^m_{i=1} dist^2(X_i, \mathcal{C}) \geq \sum^m_{i=1}dist^2(X_i^f,\mathcal{C}^f)
\label{eq:error-fdist}
\end{equation}
where $X^f$ and $C^f$ are projections of $X$ and $\mathcal{C}$ onto subspace $f$ respectively. \\
Since subspace $f$ is a solution to the fair loss-fair $k$-means, we know:
\begin{equation}
|B|\norm{A-A^f}^2_F = |A|\norm{B-B^f}^2_F
\label{eq:error-fair}
\end{equation}
where $A^f$ and $B^f$ are projections of $A$ and $B$ onto subspace $f$. We also know:
\begin{equation}
\norm{A-A^{SVD}}^2_F + \norm{B-B^{SVD}}^2_F \leq \norm{A-A^f}^2_F + \norm{B-B^f}^2_F
\label{eq:error-svd}
\end{equation}
where $A^{SVD}$ and $B^{SVD}$ are projections of $A$ and $B$ onto $X$'s optimal $k$-rank approximation. Projected on $X$'s optimal $k$-rank approximation, we assume error for group $A$ is smaller than group $B$'s:
\begin{equation}
|B|\norm{A-A^{SVD}}^2_F \leq |A|\norm{B-B^{SVD}}^2_F
\label{eq:error-assum}
\end{equation}
Subtracting equation \ref{eq:error-fair} from \ref{eq:error-assum}:
\begin{equation}
|B|\norm{A-A^{SVD}}^2_F - |B|\norm{A-A^f}^2_F \leq |A|\norm{B-B^{SVD}}^2_F - |A|\norm{B-B^f}^2_F
\label{eq:error-svdf}
\end{equation}
Adding equation \ref{eq:error-svd} times $|A|$ to equation \ref{eq:error-svdf}:
\begin{equation}
(|A|+|B|)\norm{A-A^{SVD}}^2_F < (|A|+|B|)\norm{A-A^f}^2_F \Rightarrow \norm{A-A^{SVD}}^2_F < \norm{A-A^f}^2_F
\label{eq:error-a}
\end{equation}
Given equation \ref{eq:error-a}, we conclude:
\begin{equation}
\norm{B-B^{SVD}}^2_F \geq \norm{B-B^f}^2_F
\label{eq:error-b}
\end{equation}
otherwise, projecting onto $X$'s $k$-rank approximation would result in a lower loss for both groups $A$ and $B$, which  contradicts subspace $f$ being a valid solution to the error-fair $k$-means problem.\\
We also know that the optimal solution to $K$-means clustering problem, $Z$, is an upper bound for the error of $X$ with respect to its $k$-rank approximation:
\begin{equation}
Z \geq \norm{X-\hat{X}}^2_F = \norm{A-A^{SVD}}^2_F + \norm{B-B^{SVD}}^2_F
\end{equation}
Therefore, the cost of projection compared to optimal clustering would be:
\begin{align}
\norm{B-B^f}^2_F + \norm{A-A^f}^2_F &\leq \norm{B-B^{SVD}}^2_F + \norm{A-A^f}^2_F \\
&= \norm{B-B^{SVD}}^2_F + \frac{|A|}{|B|} \norm{B-B^f}^2_F \\
& \leq (1+\frac{|A|}{|B|})\norm{B-B^{SVD}}^2_F \\
& \leq (1+\frac{|A|}{|B|})Z \label{eq:error-proj}
\end{align}
Considering a solution $Z^f$ in the error-fair subspace, given equations \ref{eq:error-fdist} and \ref{eq:error-proj} we have:
\[Z^f = \sum^m_{i=1}dist^2(X_i^f,\mathcal{C}^f) + \norm{B-B^f}^2_F + \norm{A-A^f}^2_F \leq (2+\frac{|A|}{|B|})Z\]

\end{proof}


\begin{defn} (Loss). 
Given a matrix $Y$, let $\hat{Y}$ be the optimal rank-$d$ approximation of $Y$. For a matrix $X$ with rank at most $k$, loss is defined:
\[loss(Y,X) \coloneqq \norm{Y-X}^2_F - \lVert Y-\hat{Y} \rVert^2_F \]
\end{defn}

\begin{defn}(Loss-fair $k$-means - Fair PCA). 
Given a set of data points with two subgroups $A$ and $B$, the problem of fair $k$-means with respect to loss, is defined as optimizing:
\[\argmin_{f: rank(f)\leq k} max\{\frac{1}{|A|}loss(A,A^f),\frac{1}{|B|}loss(B,B^f)\}\]
where $A^f$ is the projection of $A$ onto $f$.
\end{defn}


\begin{thm}
Let $f$ be solution to the loss-fair $k$-means problem. Then:
\[\frac{1}{|A|}loss(A,A^f) = \frac{1}{|B|}loss(B,B^f)\]
\end{thm}
\begin{proof}
Refer to the proof of \ref{th:equal}.
\end{proof}

\begin{thm}
Given a set of data points $X \in \mathbb{R}^{m \times n}$, solving the $k$-means clustering problem on the projection of $X$ onto a loss-fair subspace $f: rank(f) \leq k$, returns a $2+\frac{|A|}{|B|}$-approximate solution.
\end{thm}
\begin{proof} Since subspace $f$ is a solution to the loss-fair $k$-means, we know:
\begin{equation}
|B|\norm{A-A^f}^2_F - |B|\norm{A-\hat{A}}^2_F = |A|\norm{B-B^f}^2_F - |A|\norm{B-\hat{B}}^2_F
\label{eq:fair}
\end{equation}
where $A^f$ and $B^f$ are projections of $A$ and $B$ onto subspace $f$ and $\hat{A}$ and $\hat{B}$ are $A$ and $B$'s optimal rank $k$ approximations respectively. Projected on $X$'s optimal $k$-rank approximation, we assume loss for group $A$ is smaller than group $B$'s:
\begin{equation}
|B|\norm{A-A^{SVD}}^2_F - |B|\norm{A-\hat{A}}^2_F \leq |A|\norm{B-B^{SVD}}^2_F - |A|\norm{B-\hat{B}}^2_F
\label{eq:assum}
\end{equation}
Subtracting equation \ref{eq:fair} from \ref{eq:assum}:
\begin{equation}
|B|\norm{A-A^{SVD}}^2_F - |B|\norm{A-A^f}^2_F \leq |A|\norm{B-B^{SVD}}^2_F - |A|\norm{B-B^f}^2_F
\label{eq:svdf}
\end{equation}
Adding equation \ref{eq:error-svd} times $|A|$ to equation \ref{eq:svdf}:
\begin{equation}
(|A|+|B|)\norm{A-A^{SVD}}^2_F < (|A|+|B|)\norm{A-A^f}^2_F \Rightarrow \norm{A-A^{SVD}}^2_F < \norm{A-A^f}^2_F
\label{eq:a}
\end{equation}
Given equation \ref{eq:a}, we conclude:
\begin{equation}
\norm{B-B^{SVD}}^2_F \geq \norm{B-B^f}^2_F
\label{eq:b}
\end{equation}
As was the case for the error-fair $k$-means. The rest of the proof follows the proof for Theorem \ref{th:error-fair}.\\
\end{proof}

%Since it is possible that:
%\[\norm{B-\hat{B}}^2_F = \norm{A-\hat{A}}^2_F = \norm{A-A^{SVD}}^2_F = 0\]
%in equation \ref{eq:abneq}, a better approximation result for fair clustering problem may not be achievable (if the 2-approximation result for regular clustering problem is tight).\\

With the assumption that loss for group $A$ is smaller than group $B$'s, $2+\frac{|A|}{|B|}$ approximation reveals an interesting property of loss-fair clustering. Loss-fair $k$-means aims to minimize the maximum value of \emph{average} loss; which results in an equal average loss for the two given groups. However, when $A$ and $B$ vary in size greatly, the cost of fair K-Means clustering could become much higher than the cost of regular K-Means clustering. This means that no matter how small group $B$ might be, in order to ensure a fair outcome,  the whole population must suffer a greater  loss on average compared to the optimal solution.


\begin{defn} (Ratio). 
Given a matrix $Y$, let $\hat{Y}$ be the optimal rank-$k$ approximation of $Y$. For a matrix $X$ with rank at most $k$, ratio is defined:
\[ratio(Y,X) \coloneqq \frac{\norm{Y-X}^2_F}{\norm{Y-\hat{Y}}^2_F}\]
\end{defn}

\begin{defn}(Ratio-fair $k$-means). 
Given a set of data points with two subgroups $A$ and $B$, the problem fair $k$-means with respect to ratio, is defined as optimizing:
\[\argmin_{f: rank(f)\leq d} max\{ratio(A,A^f),ratio(B,B^f)\}\]
where $A^f$ is the projection of $A$ onto $f$.
\end{defn}

\begin{thm}
Given a set of data points $X \in \mathbb{R}^{m \times n}$, solving the $k$-means clustering problem on the projection of $X$ onto a ratio-fair subspace $f: rank(f) \leq k$, returns a $1+\frac{\norm{B-B^f}^2_F}{\norm{B-\hat{B}}^2_F}$-approximate solution.
\end{thm}

\begin{proof}
Since subspace $f$ is a solution to ratio-fair $k$-means, we know:
\begin{equation}
\frac{\norm{A-A^f}^2_F}{\norm{A-\hat{A}}^2_F} = \frac{\norm{B-B^f}^2_F}{\norm{B-\hat{B}}^2_F}
\label{eq:ratio-eq}
\end{equation}
Also, Equation \ref{eq:error-svd} still holds, therefore:
\[\norm{B-B^f} \leq \norm{B-B^{SVD}} , \norm{A-A^f} \geq \norm{A-A^{SVD}}\]
because otherwise, projecting onto $X$'s $k$-rank approximation would result in a lower loss for both groups $A$ and $B$, which  contradicts subspace $f$ being a valid solution to the ratio-fair $k$-means problem. Knowing Equation \ref{eq:ratio-eq}, we can provide an approximation to a ratio-fair solution $Z^f$:
\begin{align*}
Z^f &= \sum^m_{i=1}dist^2(X_i^f,\mathcal{C}^f) + \norm{B-B^f}^2_F + \norm{A-A^f}^2_F \\
&\leq Z + \norm{B-B^{SVD}}^2_F + \frac{\norm{B-B^f}^2_F}{\norm{B-\hat{B}}^2_F}\norm{A-\hat{A}}^2_F \\
&\leq Z + \norm{B-B^{SVD}}^2_F + \frac{\norm{B-B^f}^2_F}{\norm{B-\hat{B}}^2_F}\norm{A-A^{SVD}}^2_F \\
&\leq Z + \frac{\norm{B-B^f}^2_F}{\norm{B-\hat{B}}^2_F}Z = (1+\frac{\norm{B-B^f}^2_F}{\norm{B-\hat{B}}^2_F})Z
\end{align*} 
\end{proof}


\section{$k$-median}
Given a set of data points $\mathcal{X}$, the goal in the metric $k$-median problem is to open a set of at most $k$ centers as to minimize the sum of the distances from each data point $x_i \in \mathcal{X}$ to its nearest center. Assuming $cost(i,j)$ represents the cost (distance) between point $x_i$ and center $c_j$, we can formulate the $k$-median problem as an integer program:
\begin{equation}
\begin{array}{ll@{}ll}
\text{minimize}  & \displaystyle \sum_{j \in \mathcal{C}}\sum_{i \in \mathcal{X}} c(i,j)x_{ij} &\\
\text{subject to}& \displaystyle \sum_{j \in \mathcal{C}} x_{ij} \geq 1   &\forall i \in \mathcal{X}\\
				 & \displaystyle \sum_{j \in \mathcal{C}} y_j \leq k &\\
				 & x_{ij} \leq y_j & \forall i \in \mathcal{X}, j \in \mathcal{C}\\
                 & x_{ij},y_j \in \{0,1\} & \forall i \in \mathcal{X}, j \in \mathcal{C}
\end{array}
\end{equation}
where $y_j = 1$ if center $c_j$ is selected and $x_{i,j} = 1$ if point $x_i$ is assigned to center $c_j$. The LP relaxation of this formation allows for variables $x_{ij}$ and $y_j$ to take fractional non-negative values. A closely related problem is \emph{facility location problem} where a cost $f(j)$ is assigned for opening facility (center) $c_j$. The goal in facility location problem is to open a set of facilities so that the sum of distances from each client (point) to its nearest facility (center) plus total cost of opening facilities is minimized. Linear program formulation of facility location problem is: 
\begin{equation}
\begin{array}{ll@{}ll}
\text{minimize}  & \displaystyle \sum_{j \in \mathcal{C}}\sum_{i \in \mathcal{X}} c(i,j)x_{ij} + \sum_{j \in \mathcal{C}}f(j)y_j &\\
\text{subject to}& \displaystyle \sum_{j \in \mathcal{C}} x_{ij} \geq 1   &\forall i \in \mathcal{X}\\
				 & x_{ij} \leq y_j & \forall i \in \mathcal{X}, j \in \mathcal{C}\\
                 & x_{ij},y_j \geq 0 & \forall i \in \mathcal{X}, j \in \mathcal{C}
\end{array}
\label{eq:facilitylp}
\end{equation}
Jain et al. observed that a Lagrangian relaxation of the $k$-median problem is the facility location problem where all facilities have the same opening cost \citep{jain2001approximation}. With this observation, they proposed a primal-dual approach to solve the facility location problem and used it as a subroutine to solve the $k$-median problem. Dual program for \ref{eq:facilitylp} is:
\begin{equation}
\begin{array}{ll@{}ll}
\text{maximize}  & \displaystyle \sum_{i \in \mathcal{X}} \alpha_i &\\
\text{subject to}& \displaystyle \alpha_i - \beta_{ij} \leq c(i,j)   &\forall i \in \mathcal{X}, j \in \mathcal{C}\\
				 & \displaystyle \sum_{i \in \mathcal{X}} \beta_{ij} \leq f(j) &\forall j \in \mathcal{C}\\
                 & \alpha_i, \beta_{i,j} \geq 0 & \forall i \in \mathcal{X}, j \in \mathcal{C}
\end{array}
\end{equation}
If client $i$ is served by facility $j$, then the amount $\alpha_i$ paid by the client must be at least equal to $c(i,j)$ in the dual form. If $\alpha_i > c(i,j)$, the rest, $\beta_{ij} = \alpha_i-c(i,j)$, goes towards paying for the cost of opening the facility $j$. There are two phases in the algorithm proposed by Jain et al. \citep{jain2001approximation}. In the first phase, all clients raise their dual variable $\alpha_i$ at unit rate. When $\alpha_i = c(i,j)$, dual variable $\beta_{ij}$ will be raised at the same unit rate. When all clients are connected to at least one open facility ($\sum_{i \in \mathcal{X}} \beta_{ij} = f(j)$), the first phase is over. In the second phase, a subset of opened facilities is selected so no client is paying towards building more than one facility.

\subsection{Fairness approach 1}
In order to incorporate the \emph{fairness with respect to error} constraint into the solution, we can add priority to locations from the minority group in terms of \emph{demands}. Therefore, if the size of majority group is $A$ and the size of the minority group is $B$, the objective function in the primal LP is modified to:
\[\sum_{j \in \mathcal{C}}\sum_{i \in \mathcal{X}} d_i \times c(i,j)x_{ij}\]
where $d_i$ equals to $\frac{A}{A+B}$ if client $i$ is in the minority group and $\frac{B}{A+B}$ otherwise. The corresponding constraint in the dual form is then modified to:
\[ \forall j \in \mathcal{C}, i \in \mathcal{X}: \alpha_i-\beta_{ij} \leq c(i,j) \times d_i\]
The only change to the Jain et al.'s algorithm is that for each client $i$, $\alpha_i$ is raised at rate $d_i$. And once edge $(i,j)$ goes tight (satisfies the service cost $c(i,j)$), $\beta_{ij}$ will be increasing at rate $d_i$ too. So the facility $j$ is likely to be opened earlier than in the unit rate case.
%\manote{In case of fairness with respect to ratio, we set $d_i = \frac{1}{cost_{opt(B)}(B)}$ for $B$ and $d_i = \frac{1}{cost_{opt(A)}(A)}$ for $A$.}

\newpage
\subsection{Fairness approach 2}
There is another way to enforce fairness through the objective function for $k$-median:
\[\text{minimize max}(\frac{1}{A}\sum_{j \in \mathcal{C}}\sum_{i \in \mathcal{A}} c(i,j)x_{ij}, \frac{1}{B}\sum_{j \in \mathcal{C}}\sum_{i \in \mathcal{B}} c(i,j)x_{ij})\]
Writing the LP for this objective function:
\begin{equation*}
\begin{array}{ll@{}ll}
\text{minimize}  & \mu  &\\
\text{subject to}& \displaystyle \mu \geq \frac{1}{A}\sum_{j \in \mathcal{C}}\sum_{i \in \mathcal{A}} c(i,j)x_{ij} &\\
				 & \displaystyle \mu \geq \frac{1}{B}\sum_{j \in \mathcal{C}}\sum_{i \in \mathcal{B}} c(i,j)x_{ij} &\\
				 & \displaystyle \sum_{j \in \mathcal{C}} x_{ij} \geq 1   &\forall i \in \mathcal{X}\\
				 & \displaystyle \sum_{j \in \mathcal{C}} y_j \leq k &\\
				 & x_{ij} \leq y_j & \forall i \in \mathcal{X}, j \in \mathcal{C}\\
                 & x_{ij},y_j \geq 0 & \forall i \in \mathcal{X}, j \in \mathcal{C}
\end{array}
\end{equation*}
Equivalent LP for facility location problem would be:
\begin{equation*}
\begin{array}{ll@{}ll}
\text{minimize}  & \mu  &\\
\text{subject to}& \displaystyle \mu \geq \frac{1}{A}\sum_{j \in \mathcal{C}}\sum_{i \in \mathcal{A}} c(i,j)x_{ij} + \frac{1}{A}\sum_{j \in \mathcal{C}}f(j)y_j &\\
				 & \displaystyle \mu \geq \frac{1}{B}\sum_{j \in \mathcal{C}}\sum_{i \in \mathcal{B}} c(i,j)x_{ij} + \frac{1}{B}\sum_{j \in \mathcal{C}}f(j)y_j &\\
				 & \displaystyle \sum_{j \in \mathcal{C}} x_{ij} \geq 1   &\forall i \in \mathcal{X}\\
				 & x_{ij} \leq y_j & \forall i \in \mathcal{X}, j \in \mathcal{C}\\
                 & x_{ij},y_j \geq 0 & \forall i \in \mathcal{X}, j \in \mathcal{C}
\end{array}
\end{equation*}





\section{$k=1$}
Assume we have two groups $A$ and $B$ in the population. We add the fairness constraint-equality of average distance to center across groups-to the cost function:
\[\sum_{u_i \in A}(c-u_i)^2 + \sum_{v_i \in B}(c-v_i)^2 + \lambda(\frac{\sum_{v_i \in B}(c-v_i)^2}{|B|} - \frac{\sum_{u_i \in A}(c-u_i)^2}{|A|})\]
where $c$ is the cluster center and $\lambda$ is the trade-off parameter. We also assume group $B$ has the larger average cost between the two groups. To find the value for $c$ which minimizes the cost function, we find its derivative's root:
\[
\frac{\partial}{\partial c}\sum_{u_i \in A}(c-u_i)^2 + \sum_{v_i \in B}(c-v_i)^2 + \lambda(\frac{\sum_{v_i \in B}(c-v_i)^2}{|B|} - \frac{\sum_{u_i \in A}(c-u_i)^2}{|A|}) = 0
\]
taking the derivative:
\begin{align*}
0 &= \sum_{u_i \in A}(c-u_i) + \sum_{v_i \in B}(c-v_i) + \frac{\lambda}{|B|}\sum_{v_i \in B}(c-v_i) - \frac{\lambda}{|A|}\sum_{u_i \in A}(c-u_i) \\
&= (1+\frac{\lambda}{|B|})\sum_{v_i \in B}(c-v_i) + (1-\frac{\lambda}{|A|})\sum_{u_i \in A}(c-u_i)\\
&= (|B| + \lambda)c - \frac{|B| + \lambda}{|B|}\sum_{v_i \in B}v_i + (|A|-\lambda)c - \frac{|A| - \lambda}{|A|}\sum_{u_i \in A}u_i \\
\end{align*} 
therefore:
\[c = \frac{\frac{|B| + \lambda}{|B|}\sum_{v_i \in B}v_i + \frac{|A| - \lambda}{|A|}\sum_{u_i \in A}u_i}{|A|+|B|}\]

%\section{Fairness in Spectral Clustering}
The input in a given clustering problem, could also be modeled as a similarity graph: The
weight of an edge $w_{ij}$, represents the similarity of the vertices (points) $i$ and $j$. This similarity graph, would have large weights on the edges between two vertices corresponding to two points that are close together and small weights for points that are far apart. 

A clustering algorithm performs well if points that are similar are assigned the same cluster and points that are dissimilar are assigned to different clusters. Informally, in a similarity graph setting, this translates to partitioning vertices in a way so the sum of inter-cluster edge-weights is relatively small while the sum of edge-weights within the clusters is large. A quantity that is useful to measure this objective is \emph{conductance}. The conductance of a cut $(S,\bar{S})$ in graph $G=(V,E)$ is denoted by:
\[\phi(S) = \frac{\sum_{i \in S, j \notin S}w_{ij}}{min\{a(S),a(\bar{S})\}}\]
where:
\[a(S) = \sum_{i\in S}\sum_{j \in V}a_{ij}\]

Adopting conductance as the notion to optimize for, one of the algorithms which empirically performs well on similarity graphs in a number of applications, is spectral clustering. In Figure \ref{fig:spectral}, cut $B$ results in $\frac{5}{13}$ conductance, which is the minimum value over all the possible cuts in this graph. 

Given this notion, a desired property for each individual vertex could be defined as its \emph{in cluster connectedness} to the other vertices within the same cluster. Returning to the example graph in Figure \ref{fig:spectral}, the cut which preserves the highest amount of connections for black vertices is $B$, which also happens to be the optimal cut with respect to conductance. However cut $A$, though it's not the optimal cut, preserves the highest amount of connections for red vertices. A fair spectral clustering algorithm could be defined as:
\begin{defn}(Fair Spectral Clustering). 
Given a similarity graph with vertices partitioned into two subgroups $A$ and $B$, we define the problem of fair Spectral clustering as finding a $k$-partitioning on the vertex set, so the average loss in in cluster connectedness for the two groups is equal. 
\end{defn}
\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{spectral.pdf}
\caption
{Cut $B$ minimizes conductance while cut $A$ is intuitively more fair to red vertices.}    
\label{fig:spectral}
\end{figure}

